Measuring Distributional Shifts in Text: The Advantage of Language Model-Based Embeddings

An essential part of monitoring machine learning models in production is measuring input and output data drift. In this paper, we present a system for measuring distributional shifts in natural language data and highlight and investigate the potential advantage of using large language models (LLMs) for this problem. Recent advancements in LLMs and their successful adoption in different domains indicate their effectiveness in capturing semantic relationships for solving various natural language processing problems. The power of LLMs comes largely from the encodings (embeddings) generated in the hidden layers of the corresponding neural network. First we propose a clustering-based algorithm for measuring distributional shifts in text data by exploiting such embeddings. Then we study the effectiveness of our approach when applied to text embeddings generated by both LLMs and classical embedding algorithms. Our experiments show that general-purpose LLM-based embeddings provide a high sensitivity to data drift compared to other embedding methods. We propose drift sensitivity as an important evaluation metric to consider when comparing language models. Finally, we present insights and lessons learned from deploying our framework as part of the Fiddler ML Monitoring platform over a period of 18 months.

==> 7-related-work.tex <==
Detecting changes in the features or model outputs and verifying the validity of model inputs is a longstanding problem in ML. Here, we give a background on the techniques as well as tools available that address this problem.

Some of the simplest techniques to verify feature validity involve adding user-defined tests. For instance, \cite{schelter2018automating} suggests adding tests to verify the minimum / maximum of input features to the model. More complex tests like comparing the histogram of the feature can also be added. On the plus side, these tests are easily interpretable due to their simplicity. However, they may require a large configuration overhead from the user.

Drift detection can be posed as a null hypothesis significance testing (NHST) problem: Given two sets of samples, check via a test statistic (e.g., mean) if the two samples come from the same distribution. Some of the most well-known tests are Student's t-test and Kolmogorov–Smirnov test~\cite{wasserman2004all,murphy2012machine}. For higher dimensional data, more advanced tests, for instance, Maximum Mean Discrepancy can also be used~\cite{gretton2012kernel}. However, these tests require more fine-tuning (e.g., selecting the kernel and its hyperparameters). Confidence intervals offer an alternative to performing NHST. 
In \modelmonitor/, we leverage bootstrap based confidence intervals for detecting drifts~\cite{efron1994introduction}.

Several open source and commercial tools provide users with the ability to monitor predictions of deployed ML models, e.g., Deequ \cite{schelter2018automating}, Evidently \cite{evidently}, Fiddler's  Explainable Monitoring \cite{fiddler_monitor}, Google Vertex AI Model Monitoring \cite{google_drift}, IBM Watson OpenScale \cite{ibm_monitor}, Microsoft Azure MLOps \cite{azure_monitor}, and Uber's Michelangelo platform~\cite{uber_michelangelo}.


%Several deployed systems also provide users with the ability to monitor predictions of ML models. For instance, Uber's Michelangelo platform~\cite{uber_michelangelo} provides the statistics computed over the model predictions, optionally joining the predictions with observed outcomes (that become available later) to compute accuracy-style metrics, and allowing users to set threshold on the value of these metrics over time to raise alerts.  Similarly, Microsoft Azure~\cite{azure_monitor}, Google Cloud Platform~\cite{google_drift}, IBM Cloud~\cite{ibm_monitor}, Fiddler's ML Monitoring~\cite{fiddler_monitor}, and TruEra Monitoring~\cite{truera_monitor} offer monitoring capabilities for deployed ML models.


\modelmonitor/ detects potential  performance degradation in a model-agnostic manner and without needing to store the full training dataset. However, specialized solutions that leverage the model internals and the training data can be used to quantify the extent of drift and take targeted corrective actions (e.g.,~\citet{NEURIPS2020_219e0524,lipton2018detecting,reddi2015doubly,wu2019domain}). Due to their model and data introspective nature, these solutions are beyond the scope of this paper.


==> back-3-modelmonitor-design-and-architecture.tex <==
\subsection{Key Requirements}
We next summarize key design requirements, gathered from customers and domain experts, that were used to shape \modelmonitor/.

{\bf Be accessible:} Model monitoring is a key part of the ML lifecycle and a critical MLOps component: it should be approachable by customers with any level of expertise, both in terms of engineering and ML. There should be minimal amount of code needed to get started, and it should provide sensible defaults where possible. However, it should not preempt more advanced use cases.

{\bf Be scalable:} Frequently used models in production settings can generate large amounts of data. Processing this data should not impact inference; additionally the analysis has to be fast and scale horizontally.
    
{\bf Handle historical data:} Analysis is done not only on the most recent data but on historical data as well. This data, a sample of it, or its summary should be stored in a way that is securely and readily accessible.
    
{\bf Incorporate external sources:} Analysis often requires not only model inputs and outputs but external sources such as labels that may only be known with some delay after inference itself. It should be easy to quickly access the inference traffic data together with its corresponding labels or other external information.

\subsection{\modelmonitor/ Architecture} \label{sec:components}
\modelmonitor/ consists of three major components: data analysis, data collection, and scheduling.

\subsubsection{Data Analysis \label{data_analysis}}
The data analysis component strives to achieve these design goals:
(1) scale to any amount of inference data, (2) provide sensible defaults for ease of use, and (3) provide an interface that can be easily and intuitively extended (for instance by scientists or domain experts), e.g.,\ allowing custom metrics.

\modelmonitor/ performs data analysis by leveraging SageMaker Processing,\footnote{\scriptsize \url{https://docs.aws.amazon.com/sagemaker/latest/dg/processing-job.html}} a scalable cloud platform for ETL workloads. The data analysis component contains the core analysis logic and is packaged as a Docker image for use in SageMaker Processing. Users with different analysis needs have the option of providing a custom
Docker image.
SageMaker Processing runs customer-defined analyses by loading Docker images: for some metrics we turned to proven open-source technologies to drive the core analysis logic, using amongst others, Apache Spark MLlib and Deequ \cite{schelter2018automating}. In some cases, we contributed back to open source projects, e.g., by extending the functionality of Deequ allowing it to track an approximate histogram of the data.
Our use of Apache Spark and S3 for data collection allows us to easily distribute the load amongst instances provisioned by SageMaker Processing, and scale as needed.

Upon startup, the analyzer loads relevant inference data, as well as labeled data (when applicable),
and produces a time-bound analysis. It computes a standard set of metrics by default, which we describe in depth in \S\ref{sec:methodology}. We show a sample generated report in Appendix \ref{app:samplereport}.

We support custom analyses as follows.
For use cases where our default metrics are not a good fit, a custom Docker image can be provided. Note that, in this scenario, the analysis is still run on the data collected through our Data Collection system described in \S\ref{data_collection}. If however, small changes prior to analysis are required, pre-processing (run over each row) and post-processing (run after analysis is done) Python hooks are provided. While our analysis is done in Spark, we chose to provide hooks in Python due to its popularity in the ML community.


\subsubsection{Data Collection \label{data_collection}}
SageMaker Endpoints is a fully-managed real-time model hosting platform. As part of \modelmonitor/, we built a data collection (also referred to as data capture) component to (1) capture and collect the inputs and outputs sent to these Endpoints
and (2) a way to join this data with external signals such as labels/annotations.

The first part operates with no code change on the Endpoints as it captures only inputs and outputs, and not intermediate data. This is crucial for ease of use, especially for already existing systems that wish to start using \modelmonitor/. See Appendix \ref{app:enabling} for details into this area. Other than ease of use, our main focus for data collection was to avoid impact to inference workloads: extraneous resource usage (CPU, memory, disk, network) must be minimal.

Minimizing resource usage is a well studied problem in logging systems. We approached this problem in two stages: (1) requests and responses are saved to disk in a format that is easy to break up (JSON lines),  and (2) a daemon polls the disk for changes - upon reaching thresholds for size and time between uploads, the daemon initiates the transfer into S3. 
For ease of analysis, we store the data in sub-folders structured as yyyy/mm/dd/hh. Further, we exclusively use UTC timestamps to avoid confusion related to multiple time zones and non-existing hours due to daylight savings time changes.

Stage (2) above is required for tracking performance metrics such as accuracy. To use it, users are responsible for adding an identifier in each inference request, which gets saved in S3 along with the rest of the data. They must then emit the ground truth label or value into S3 in the same hourly sub-folder format we use for inference requests, each with the corresponding identifier. 

\subsubsection{Scheduling \label{scheduler}}

This component controls the orchestration between the inference nodes and other \modelmonitor/ components. 
In particular, this component allows users to configure the analysis hardware (e.g., size and number of instances) and frequency.

For simplicity, \modelmonitor/ performs analyses in hourly batches. This was a coarse enough granularity to provide a sensible way to store in S3, but granular enough to provide a useful signal upon analyzing the data. Storing the data in this manner meant, however, that analysis was constrained to run at the top of the hour, if we wanted to analyze the preceding hour's data as soon as possible. Implementing this approach naively would cause imbalance in terms of compute. Our solution was to add a random delay to each job of up to twenty minutes, which spreads jobs more evenly and 
avoids overloading our service at the top of every hour.

Note that it could be possible not to persist the joined data, and instead run the analysis on it and discard it shortly after. However, to allow multiple components to perform analysis on this data - 
our own, users' custom components, and third party monitoring tools
- we found it to be a better design choice to have a separate job for joining the data as well as persisting it in S3. The scheduler runs this ``join'' job before running the analysis that requires the data.


\subsection{Integration with Amazon SageMaker} \label{architecture}


\modelmonitor/ was built to provide an integrated and seamless experience for customers of SageMaker and Amazon Web Services. As shown in Fig.~\ref{architectureDiagram} and described in the preceding section, \modelmonitor/ is built to understand and analyze data collected by SageMaker Endpoints. The amount of data to be collected can be tuned taking into account storage and compute costs. In addition, data generated by \modelmonitor/ are stored in 
Amazon S3 (see Appendix \ref{app:samplereport} for an example),
enabling the export and use of other AWS Services to perform additional analysis on the data. \modelmonitor/ jobs also emit metrics to Amazon CloudWatch,\footnote{\scriptsize \url{https://aws.amazon.com/cloudwatch/}} a monitoring service, to indicate whether a deviation in quality was identified. Users can set alarms on these metrics to alert operators, who can then take remedial action. For instance, an operator may realize, upon seeing a ``mismatched number of columns alert'' that an upstream service is no longer one-hot encoding a feature. In such a scenario, reverting the deployment may be the most expedient course of action.



\begin{figure}[t]
\centering
  \includegraphics[width=\columnwidth]{figures/arch_diagram.png}
  \caption{High-level system architecture of \modelmonitor/}
  \label{architectureDiagram}
\end{figure}

